System identification of a hysteresis-controlled pump system using SINDy

Hysteresis-controlled devices are widely used in industrial applications. For example, cooling devices usually contain a two-point controller, resulting in a nonlinear hybrid system with two discrete states. Dynamic models of systems are essential for optimizing such industrial supply technology. However, conventional system identification approaches can hardly handle hysteresis-controlled devices. Thus, the new identification method Sparse Identification of Nonlinear Dynamics (SINDy) is extended to consider hybrid systems. SINDy composes models from basis functions out of a customized library in a data-driven manner. For modeling systems that behave dependent on their own past as in the case of natural hysteresis, Ferenc Preisach introduced the relay hysteron as an elementary mathematical description. In this new method (SINDyHybrid), tailored basis functions in form of relay hysterons are added to the library which is used by SINDy. Experiments with a hysteresis controlled water basin show that this approach correctly identifies state transitions of hybrid systems and also succeeds in modeling the dynamics of the discrete system states. A novel proximity hysteron achieves the robustness of this method. The impacts of the sampling rate and the signal noise ratio of the measurement data are examined accordingly.

==> tank_model_variables.tex <==
\begin{table}
\captionof{table}{Parameter of the tank simulation}
	\label{table:wassertankParameter}

	%
\begin{tabular}{|m{1cm}| m{2.8cm} | m{2.3cm}|} \hline
			\textbf{Symbol}	& \textbf{Settings} & \textbf{Meaning} \\[10pt]  \hline \hline
			
$h_0$ & 15 & initial level \\[10pt]  \hline
			
$h_{max}$ &{\small $\begin{aligned} &Tr: 20, 21 \\  &Val.: 19, 19.5, 20.5, 22 \end{aligned}$} &upper boundary \\[14pt] \hline
			
$h_{min}$ & {\small $\begin{aligned} &Tra: 18, 19 \\  &Val.: 16, 18.5, 17.5, 18 \end{aligned}$} &lower boundary \\[14pt] \hline
			
inflow $z$ & {\small $\begin{aligned} &Tr: 1.2, 1.8 \\  &Val.: 1.5, 1.3, 1.7, 1.6 \end{aligned}$} & inflow \\[14pt] \hline
			
outflow $a$ & {\small $\begin{aligned} &Tr: 0.2, 0.4 \\  &Val.: 0.15, 0.25, 0.35, 0.45 \end{aligned}$} & outflow \\[14pt] \hline
			
$l_r$ & 0, 1, 5, 10, 50  & Length $u$ und $h$  \\[10pt] \hline
			
$h(t)$ & \textit{ \footnotesize dynamics}  & level \\[10pt] \hline
			
$u(t)$ & \textit{ \footnotesize dynamics}  & pump control  \\[10pt] \hline
\end{tabular}
	
\end{table}

